A Tale of Tails: Model Collapse as a Change of Scaling Laws

As AI model size grows, neural scaling laws have become a crucial tool to predict the improvements of large models when increasing capacity and the size of original (human or natural) training data. Yet, the widespread use of popular models means that the ecosystem of online data and text will co-evolve to progressively contain increased amounts of synthesized data. In this paper we ask: How will the scaling laws change in the inevitable regime where synthetic data makes its way into the training corpus? Will future models, still improve, or be doomed to degenerate up to total (model) collapse? We develop a theoretical framework of model collapse through the lens of scaling laws. We discover a wide range of decay phenomena, analyzing loss of scaling, shifted scaling with number of generations, the ''un-learning" of skills, and grokking when mixing human and synthesized data. Our theory is validated by large-scale experiments with a transformer on an arithmetic task and text generation using the large language model Llama2.

==> CumulativeWriteup/proofs.tex <==
\section{Proofs}
 \subsection{Proof of Theorem \ref{thm:simple}}
 Observe that the model $\widehat f$ makes an error on $i$ if and only if the $i$th "skill" never occurred in the training dataset $\mathcal D_T$, i.e either (1) $i \ge k + 1$, or (2) $1 \le i \le k$ and $i_t \ne i$ for all $t \in [T]$. We deduce that
\begin{eqnarray*}
\begin{split}
 E_{test} = \mathbb P_{i \sim p}(\widehat f(i) \ne y_i) &= \sum_{i \ge k+1}p_i + \sum_{1 \le i \le k}p_i(1-p_i)^T\\
 &\asymp k^{-(\beta-1)} + \sum_{1 \le i \le k}p_i e^{-p_i T},
 \end{split}
\end{eqnarray*}
where $c := 1-1/\beta \in (0,1)$, and we have used the elementary fact that $\sum_{i \ge k + 1}i^{-\beta} \asymp k^{-(\beta-1)}$ for large $k$. 
For the second sum, we will need the following lemma proved in the appendix.
\begin{lemma}
The following identity holds
\begin{eqnarray}
T^c \sum_{i=1}^k p_i e^{-T p_i} \asymp \Gamma(c,Tk^{-\beta})-\Gamma(c,T) = O(1),
\end{eqnarray}
 where $\Gamma(s,x) := \int_x^\infty u^{s-1}e^{-u}\mathrm{d}u$ defines the incomplete gamma function. In particular, for $k=\infty$ and large $T$, it holds that $\sum_{i=1}^\infty p_i e^{-T p_i} \asymp T^{-c}$.
\label{lm:gamma}
\end{lemma}
 We now consider two separate cases for the relative scaling of $k$ and $T$.
 
 \paragraph{-- Case 1: $T \gtrsim k^\beta$.}
 Here, we have thanks to Lemma \ref{lm:gamma}
 \begin{eqnarray}
     \begin{split}
 E_{test} &\asymp k^{-(\beta-1)} + O(T^{-c}) \asymp k^{-(\beta-1)},
     \end{split}
 \end{eqnarray}
since $k^{-(\beta-1)} \gtrsim T^{-(\beta-1)/\beta} = T^{-c}$.

 \paragraph{-- Case 2: $1 \ll T \lesssim k^\beta$.} Here, thanks to Lemma \ref{lm:gamma} we have $\Gamma(c,T) = o(1)$ and $\Gamma(c,Tk^{-\beta}) = \Theta(1)$. We deduce that
 \begin{eqnarray}
 \begin{split}
     E_{test} &\asymp k^{-(\beta-1)} + T^{-c}\left(\Gamma(c,Tk^{-\beta}) - \Gamma(c,T)\right) \asymp k^{-(\beta-1)} + T^{-c} \asymp T^{-c},
     \end{split}
 \end{eqnarray}
 since $k^{-(\beta-1)} \lesssim T^{-(\beta-1)/\beta} = T^{-c}$.
Putting things together then gives the claimed result. \qed

\subsection{Proof of Theorem \ref{thm:bigram1}}
The proof will be based on the results of \cite{Berend2012OnTC}.

 \paragraph{Upper-Bound.}
 Observe that for any choice of mappings $\pi_1,\pi_2,\ldots$, we have 
\begin{eqnarray*}
    \begin{split}
a_T(i) &:= \sum_{j\, \mid \,p(j \mid i) \le 1/n_T(i)} p(j \mid i) \asymp \sum_{j\, \mid \,\pi_i(j) \ge n_T(i)^{1/\beta}} \pi_i(j)^{-\beta} \le \sum_{k\, \mid \, k \ge n_T(i)^{1/\beta}} k^{-\beta} \asymp n_T(i)^{-(1-1/\beta)}\\
b_T(i) &:= n_T(i)^{-1/2}\sum_{j\, \mid \,p(j \mid i) \ge 1/n_T(i)} \sqrt{p(j \mid i)} \asymp n_T(i)^{-1/2}\sum_{j\, \mid \, \pi_i(j) \le n_T(i)^{1/\beta}}\pi_i(j)^{-\beta/2}\\
&\lesssim n_T(i)^{-1/2}\sum_{k\, \mid \, k \le n_T(i)^{1/\beta}}k^{-\beta/2} \asymp n_T(i)^{-c}.
    \end{split}
\end{eqnarray*}
We deduce that
$c_T(i) := a_T(i) + b_T(i) \lesssim n_T(i)^{-c}$ for any $i$.  Importantly, the hidden constants don't depend on $i$.  Therefore, thanks to \cite[Lemma 9]{Berend2012OnTC}, we have
\begin{eqnarray}
\label{eq:tvub}
\begin{split}
    E_{test} \le \sum_i p_i \mathbb E\,[c_T(i)] &\lesssim \sum_i p_i \mathbb E\,[n_T(i)^{-c}] \overset{(*)}{\le} \sum_i p_i (\mathbb E\,[n_T(i)])^{-c} = \sum_i p_i (T p_i)^{-c} = T^{-c}\sum_i p_i^{1-c}\\
    &\lesssim T^{-c},
    \end{split}
\end{eqnarray}
where we have used Jensen's inequality in (*), since the function $x \mapsto x^{-c}$ is concave.

\paragraph{Lower-Bound.} WLOG\footnote{A summable series of nonnegative numbers (like in $a_T(i)$ and $b_T(i)$) can be reordered without changing the value.} consider the following specific choice of permutations defined by $\pi_i(j) = j$ (i.e doesn't depend on $i$). Then, 
\begin{align*}
a_T(i) &= \sum_{j \ge n_T(i)^{1/\beta}} j^{-\beta} \asymp n_T(i)^{-(1-1/\beta)},
\\
b_T(i) &= n_T(i)^{-1/2}\sum_{j \le n_T(i)^{1/\beta}} j^{-\beta} \asymp n_T(i)^{-c}.
\end{align*}
Thanks to the definition of $E_{test}$ and \cite[Proposition 5]{Berend2012OnTC}, we deduce that if $\beta \in (1,2)$, then
\begin{eqnarray}
E_{test} \ge \sum_i p_i \mathbb E\,[(a_T(i) + b_T(i) - n_T(i)^{-1/2})] \asymp \sum_i p_i \mathbb E\,[n_T(i)^{-c}- n_T(i)^{-1/2})] \asymp \sum_i p_i \mathbb E\,[n_T(i)^{-c}],
\label{eq:tvlb}
\end{eqnarray}
i.e $E_{test} \gtrsim \sum_i p_i \mathbb E\,[n_T(i)^{-c}]$. Now, since $n_T(i) \sim Bin(T,p_i)$, standard Binomial concentration arguments tell us that $n_T(i) \le 1.5 T p_i$ w.p $1-e^{-Cp_i T}$, where $C$ is an absolute constant. We deduce
\begin{eqnarray*}
\begin{split}
    E_{test} &\gtrsim \sum_i p_i (1.5 T p_i)^{-c}(1-e^{-Cp_iT})\asymp T^{-c} \sum_i p_i^{1-c} - T^{-c} \underbrace{\sum_i p_i^{1-c} e^{-Cp_iT}}_{o(1)} \asymp T^{-c},
    \end{split}
\end{eqnarray*}
which completes the proof. \qed

\subsection{Proof of Theorem \ref{thm:bigram3}}
It suffices to replace $n_T(i)$ in \eqref{eq:tvub} and \eqref{eq:tvlb} of the proof of Theorem \ref{thm:bigram1} with $n_T(i) \land k^\beta$, and use the elementary fact that $(n_T(i) \land k^\beta)^{-c} = n_T(i)^{-c} \lor k^{-\beta c} \asymp n_T(i)^{-c} + k^{-\beta c}$. The rest of the proof proceeds as that of Theorem \ref{thm:bigram1}. % and \ref{thm:bigram2}.


\subsection{Proof of Theorem \ref{thm:generalcov}}
Note that $A_1 \Delta w_1 \overset{D}{=} (X^\top X + \lambda I_d)^{-1} X^\top X (X_0^\top X_0)^{-1} X_0^\top E_0$, where $E_0$ is a $T_0$-dimensional random vector with iid entries from $N(0,\sigma_0^2)$, and $X_0$ is a random $T_0 \times d$ matrix with iid rows from $N(0,\Sigma)$.

\begin{eqnarray*}
    \begin{split}
\mathbb E\,\mathrm{tr}((X_0^\top X_0)^{-1} A_n\Sigma A_n)
&=  \mathbb E\, \mathrm{tr}((X_0^\top X_0)^{-1} X^\top X(X^\top X + \lambda I_d)^{-1} \Sigma (X^\top X + \lambda I_d)^{-1} X^\top X)\\
&\cong  \frac{\phi_0}{1-\phi_0} \mathbb E\, \overline{\mathrm{tr}}(\Sigma^{-1} X^\top X(X^\top X + \lambda I_d)^{-1} \Sigma (X^\top X + \lambda I_d)^{-1} X^\top X),
    \end{split}
\end{eqnarray*}
as claimed.
\qed

In the last step of the above proof, we have used the following well-known result.
\begin{lemma}
    Let $T_0$ and $d$ be positive integers with $T_0 \ge d + 2$, and let $X_0 \in \mathbb R^{T_0 \times d}$ be a random matrix with iid rows from $N(0,\Sigma)$. Then, $X_0$ has full rank a.s. Moreover, it holds that
    \begin{eqnarray}
        \mathbb E\, [(X_0^\top X_0)^{-1}] = \frac{1}{T-d_0-1}\Sigma^{-1}.
    \end{eqnarray}
\end{lemma}
\subsection{Proof of Proposition \ref{prop:b2}}
    The first part of the result follows from applying Proposition 1 of Bach, with $A=\Sigma^{-1}$ and $B=\Sigma$.

For the second part, note that  $\mathrm{df}_m(t) = d/(1+t)^m$ and \eqref{eq:MP} holds and so
\begin{eqnarray*}
\begin{split}
    b^2 &\cong \frac{1}{(1+\kappa(\lambda))^2} + \frac{\kappa(\lambda)^2}{(1+\kappa(\lambda))^4}\frac{d}{T-\mathrm{df}_2(\kappa(\lambda))} \\
    &\cong \frac{1}{(1+\kappa(\lambda))^2} + \frac{\kappa(\lambda)^2}{(1+\kappa(\lambda))^4}\frac{\phi}{1-\phi/(1+\kappa(\lambda))^2}\\
    &= \frac{1}{(1+\kappa(\lambda))^2} + \frac{\phi\kappa(\lambda)^2}{(1+\kappa(\lambda))^2}\frac{1}{(1+\kappa(\lambda))^2-\phi},
    \end{split}
\end{eqnarray*}
as claimed. \qed

\subsection{Proof of Lemma \ref{lm:gamma}}
Consider the function $h(z) := z e^{-Tz}$ for $z \in (0,1)$. Its derivative is $h'(z) = e^{-Tz}(1-Tz)$. Thus, $h$ is increasing on $(0, 1/T)$ and decreasing on $(1/T,\infty)$. Furthermore, note that $p_i \le 1/T$ iff $i \ge T^{1/\beta}$. We deduce that
$$
\sum_{i=1}^k p_i e^{-Tp_i} \asymp \int_1^k x^{-\beta} e^{-T x^{-\beta}}\mathrm{d}x.
$$

Under the change of variable $u=u(x):=Tx^{-\beta}$, we have $x=x(u)=(u/T)^{-1/\beta}$ and so $\mathrm{d}x = -(T^{1/\beta} u^{-1-1/\beta} / \beta)\mathrm{d}u$. Also $u(1)=T$ and $u(k) = Tk^{-\beta}$. We deduce that
\begin{align*}
 \sum_{i=1}^k p_i e^{-Tp_i} &\asymp \int_1^k x^{-\beta} e^{-T x^{-\beta}}\mathrm{d}x =  \int_{Tk^{-\beta}}^T (u/T) e^{-u}(T^{1/\beta} u^{-1-1/\beta} / \beta)\mathrm{d}u\\
 &\asymp T^{-(1-1/\beta)}\int_{Tk^{-\beta}}^T u^{-1/\beta} e^{-u}\mathrm{d}u\\
 &\asymp T^{-(1-1/\beta)}\left(\Gamma(1-1/\beta,Tk^{-\beta}) - \Gamma(1-1/\beta,T)\right)\\
 &= T^{-c}\left(\Gamma(c,Tk^{-\beta}) - \Gamma(c,T)\right),
 \end{align*}
 and we are done for the first part.

 For the second part, note that $\Gamma(c,T) = o(1)$ for large $T$ so that
 $$
 (\Gamma(c,Tk^{-\beta}) - \Gamma(c,T))|_{k=\infty} = \Gamma(c,0) - \Gamma(c,T) = \Theta(1) - o(1) = \Theta(1),
 $$
 from which the result follows. \qed


\section{Technical Lemmas}
The following lemma will be useful somewhere, somehow. It is a consequence of \cite{Berend2012OnTC}.
\begin{lemma}
\label{lm:berend}
    Let $p$ be a Zipf law with exponent $\beta > 1$ and let $\widehat p_T = T^{-1}\sum_{t=1}^T \delta_{i_t}$ be an empirical estimate thereof, based on $T$ iid samples $i_1,\ldots,i_T$ from $p$. Then, it holds w.p $1-e^{-T^{\Omega(1)}}$ that $TV(\widehat p_T, p) \lesssim T^{-c}$, where $c \in (0,1/2]$ is given by
    \begin{equation}
        c=
        \begin{cases}
            1-1/\beta,&\mbox{ if }1 < \beta < 2,\\
            1/2,&\mbox{ if }\beta > 2.
        \end{cases}
    \end{equation}
    Moreover, it holds that $\mathbb E\, [TV(\widehat p_T,p)] \gtrsim T^{-c}$.
\end{lemma}
Note that in particular, the above result ensures that 
\begin{eqnarray}
\mathbb E\,[TV(\widehat p_T,p)] \asymp T^{-c}.
\end{eqnarray}
\begin{proof}
Define $a_T := \sum_{p_i < 1 / T} p_i$ and $b_T := T^{-1/2}\sum_{p_i \ge 1/T} \sqrt {p_i}$. Then, $a_T + b_T = o(1)$ for large $T$, and moreover, Theorem 4 and Proposition 5 of \cite{Berend2012OnTC} assure that $\mathbb E\,[TV(\widehat p_T, p)] \ge a_T + b_T - T^{-1/2}$, and w.p $1-e^{-T\epsilon^2/2}$, it holds that
$$
TV(\widehat p_T, p) \le a_T + b_T + \epsilon.
$$
Now, it is clear that 
\begin{align*}
    a_T &\asymp \sum_{i \ge T^{1/\beta}} i^{-\beta} \asymp \int_{T^{1/\beta}}^\infty x^{-\beta}\mathrm{d}x \asymp T^{-(\beta-1)/\beta} = T^{-(1-1/\beta)},\\
b_T &\asymp T^{-1/2}\sum_{i \le T^{1/\beta}} i^{-\beta/2} \asymp T^{-1/2} \int_1^{T^{1/\beta}}x^{-\beta/2}\mathrm{d}x\\
&\asymp T^{-1/2}\cdot \bigg[\frac{x^{1-\beta/2}}{1-\beta/2}\bigg]_{x=1}^{T^{1/\beta}}
\asymp \begin{cases}  T^{-1/2} T^{1/\beta-1/2} = T^{-(1-1/\beta)},&\mbox{ if }1 < \beta < 2,\\
T^{-1/2},&\mbox{ if }\beta > 2.
\end{cases}
\end{align*}
We deduce that $a_T + b_T \asymp T^{-c}$. The claimed upper-bound then follows upon taking $\epsilon=T^{-c}$.
\end{proof}


==> CumulativeWriteup/related.tex <==
\section{A summary of previous literature}

\julia{A reference that will allow us to relate regularization to early stopping when we need it \cite{pmlr-v89-ali19earlystop}. This can also relate to the obervation made in the Bartless self-distillation paper: early stopping is crucial for reaping the benefits in the early cycles of self-distillation.}

\julia{Missing:
\begin{itemize}
    \item Compare the Bartlett paper \cite{bartlett2020neurips} to small
    \item Compare \cite{bertrand2023stability} to our mixing results
    \item Framing of the Benefirst of synthesized data section: Depending on whether Elvis produces a bump: 1) YES -- frame all the emprics as ''they have found the bump" 2) NO - frame all the empirics as ''Big model helps little model"
\end{itemize}}

\paragraph{Model Collapse:} The phenomenon appeared in the {\em recent} literature in the context of language and image generation. Several recent works demonstrate facets of this phenomenon {\em empirically} in various settings \cite{Hataya_2023_ICCV, martínez2023combining,martínez2023understanding,bohacek2023nepotistically,briesch2023large,guo2023curious}. Only few recent works also provide some accompanying theoretical analysis \cite{shumailov2023curse,alemohammad2023selfconsuming,bertrand2023stability} which we outline now.

\cite{shumailov2023curse} define model collapse and attribute it to two mechanisms: finite sampling when training a model (leading to cut off of low-probability data) and function approximation errors (the model is not sufficiently expressive to model the true distribution). They observe (and, for a single Gaussian, prove) that upon iteratively resampling finite ''training data" the generated distribution becomes more and more peaked. Other models studied empirically are mixtures of (two) Gaussians and VAEs on MNIST. To study language models, \cite{shumailov2023curse} iteratively fine tune Meta's OPT-125M model on {\tt wikidata2}. For generation of new text they use a 5-way beam search, which, by its nature, (approximatively) generates only low-perplexity data. 

%\julia{I worry about the following statement from their paper \cite{shumailov2023curse}: {\em At the same time, we discover that generated data has much longer tails, suggesting that some of the data would never be produced by the original model – these are the errors that accumulate because of the learning with generational data.} If this is true, how can we possibly explain that? They also allude to the ''repeated text" problem of generated data, which is apparently already known.}
%\ElvisFix{Indeed, that sounds weird. I'll check their paper asap to see. Thanks for the info.}
% \ElvisIssue{Possible explanation is that: after many many generations, the generated data is straight up hallucination ? Unfortunately, we can't probe / reproduce this phenomenon using our (currently) toy LLM discrete setup (the support of the data only reduces after each generation).} \julia{What if we add some noise to the model output? But why would that generate extra tail? Truly weird. But they are very (VERY) sloppy in their paper, so maybe this just isn't reproducible. They do not observe this in the GM or VAE setting, just in their weird LLM setup.}

\julia{I commented out our chatter here, but let's keep a note on the purportedly longer tails from AI-generation (because who knows, we might be able to prove something theoretically) and mention the repeated-text problem of regenerated data.}

 \cite{alemohammad2023selfconsuming}  conduct an empirical and analytical analysis on generative image models of what they term the ''self-consuming" or ''autophaguous" loop. They conclude that without enough fresh real data at each generation, future models necessarily will have their precision or recall decrease. They model the influence of each new AI-generation via a generic {\em sampling bias} $0 \leq \lambda \leq 1 $. In the case of image generation this refers to feature parameters at generation that favor quality over diversity (suitably quantified). More precisely, $\lambda=1$ corresponds to unbiased sampling and $\lambda=0$ corresponds to sampling from the modes of the generative distribution. $\lambda$  models biased sampling methods commonly used in generative modeling practice, such as truncation in BigGAN and StyleGAN or guidance in diffusion models. 
 In the case of Gaussian distributions, $\lambda$ is the shrinking factor of the variance of the next generation. Their empirical work studies GANs and denoising diffusion probabilistic models for image generation on FFHQ and MNIST and single Gaussians for both theoretical and empirical observations. As in \cite{shumailov2023curse} they observe (and prove for the case of a single Gaussian) that estimation error alone leads to vanishing variance with number of iterations.
 \cite{alemohammad2023selfconsuming} also empirically observe an initial boost in performance in a regime where modest amounts of synthetic data are mixed with the original data before larger amounts of synthetic data lead to ultimate degradation. This might mimick larger-scale results that demonstrate how synthetic data mixed with true data improves performance in some scenarios (see {\em Benefits of synthesized data} below). Indeed, in its simplest form, data augmentation (rotations, cropping etc.~), a widespread highly beneficial practice in ML training, can be viewed as the simplest form of data generation.


A concurrent paper \cite{bertrand2023stability} on image generation \julia{Continue here.} {\em we develops a framework to rigorously study the impact of training generative models on mixed datasets (of real and synthetic data) on their stability. We first prove the stability of iterative training under the condition that the initial generative models approximate the data distribution well enough and the proportion of clean training data (w.r.t. synthetic data) is large enough. We empirically validate our theory on both synthetic and natural images by iteratively training normalizing flows and state-of-the-art diffusion models on CIFAR10 and FFHQ.} \julia{read, check and summarize.}

Several empirical studies confirm the deleterious effect of training on self-generated data: In the context of image generation, 
\cite{martínez2023combining,martínez2023understanding} report  degradation of models trained on AI-generated data. Specifically, they use a Denoising Diffusion Implicit Model and a few (relatively small) datasets (e.g.~Orchids, MNIST) to demonstrate visual degradation when training in successive generations of AI-generated data. 
\cite{Hataya_2023_ICCV} {\em ''conclude that generated images negatively affect downstream performance, while the significance depends on tasks and the amount of generated images"}, \cite{bohacek2023nepotistically} reports that the popular StableDiffusion model collapses when iteratively retrained on self-generated faces, even with as little as $3\%$ synthetic data mixed into the original training set. For text, \cite{briesch2023large} use {\em nanoGPT}\footnote{\tt https://github.com/karpathy/nanoGPT} on a curated 10K logical-expression dataset to demonstrate the iterative collapse of self-consuming loops - the model and dataset are sufficiently small to allow training from scratch. \cite{guo2023curious} observe a decline in linguistic diversity metrics across iteratively fine-tuned LLMs. 

\paragraph{Mitigation:} To our knowledge, rigorous theory (or even empirical demonstrations) on mitigation strategies against model collapse are yet to come, with one notable exception in \cite{bertrand2023stability} (see below). Several works discuss the need for {\em detection} of AI-generated images or text (to avoid retraining on them), for example motivating research into watermarking strategies. \julia{Is the following true:} Our work points to the possibility of integrating AI-generated data {\em if well curated} in particular to include the tails of the distribution. 
\cite{bertrand2023stability} analyze iterative retraining on a mixture of synthesized and original data under several assumptions \julia{continue. They seem to be the only ones to do some theory. I should ahve looked earlier. }


\paragraph{Benefits of synthesized data} There is a range of results showing benefits of AI-synthesized data in training better models, though mostly these results pertain to image data, specifically in the context of diffusion models (\cite{azizi2023synthetic,he2023is,shipard2023diversity,bansal2023leaving,lin2023explore}), though not only (see \cite{dai2023auggpt,xu2023baize,huang2022large,wang-etal-2023-self-instruct} for chat-related examples). One might argue that they either throw model-collapse caution to the winds or, possibly, settle in the protected corner where mild amounts of synthetic data (or larger amounts of ''mildly synthetic" data, like in the case of data augmentation) helps. \julia{\bf Elvis, no pressure, but we need your mixing phase transition!} \julia{A note: it seems that synthetic data helps more if it comes from a slightly shifted domain or use case. For instance, use diffusion models to produce synthetic images and then use those for classification \cite{he2023is,shipard2023diversity,bansal2023leaving,lin2023explore}. Moreover, in some cases the synthetic images come from larger or stronger models than those used in the downstream tasks, which would explain their utility (they still got most of their tails, and what has been chopped off is imperceptible to the smaller model). This is plan B in case there is no phase transition. In this case we will blame the domain shift for these ''anomalous" results.}
However, other works critically analyze the purported benefit of generated data. \cite{burg2023image} find that while synthesized data from a diffusion model helps improving downstream tasks, such as classification, using the {\em pre-training data} of the diffusion model alone gives even stronger performance (which we can interpret as evidence of mild first-generation model collapse). All in all it is fair to say that the impact of data augmentation using generative models is still not fully understood.




\paragraph{Scaling Laws:}
Neural scaling laws have been observed empirically in vision, language and speech. 

Early large scale empirical studies are performed in \cite{hestness2017deep,rosenfeld2020a}, demonstrating power law scaling across a range of learning scenarios. This is followed by  well-known large-scale studies from OpenAI
\cite{kaplan2020scaling} and DeepMind \cite{hoffmann2022trainingChinchilla}, which empirically demonstrate power-law scaling in LLMs across a wide set of scales. Essentially, this empirically establishes that 
$$L(N,D) \sim N_C\cdot N^{-\alpha_N}+D_C \cdot D^{-\alpha_D},$$ where $L$ is the per-token cross entropy loss (in nats), $N,D$ are the number of (non-embedding) parameters and data, respectively, and $N_C, D_C$ and $\alpha_N,\alpha_D$ are constants determined by the data distribution and the model specifications. 



This study was extended in a follow up \cite{henighan2021scaling}  to demonstrate many more power law relations in various scenarios (vision transformer, video modeling, multimodal models, and mathematical problem solving. In \cite{gordon-etal-2021-data}, for the machine translation (MT) setting, scaling laws for standard benchmarks like BLEU are quantified and explained via cross-entropy power-law scaling, thus positing a first universality of scaling laws across metrics. 
\cite{hernandez2021scaling} demonstrate similar empirical power-law scaling for transfer learning and \cite{aghajanyan2023scaling} provide a vast experimental body of evidence for scaling laws in mixed-modal language models.

However, a few results have nuanced the view of scaling as a panacea to improved loss. For instance, \cite{mckenzie2023inverse} present evidence for ''inverse sclaing" where flaws in the training objective or the data lead to U-shaped scaling. 

\paragraph{Theoretical models for scaling laws:} 
From a theoretical angle, scaling laws have been shown analytically even before the emergence of large foundation models. For instance, \cite{Caponnetto2007OptimalRF} characterize the power-law generalization error of regularized least-squares kernel algorithms. The role of optimization can also be taken into account in this setting (\cite{nitanda2021optimal}).
In the nonparametric literature, for example \cite{SchmidtHieber2017scaling} and \cite{suzuki2018adaptivity} derived the test error scaling of deep neural network in fitting certain target functions and \cite{BordelonCP20spectrum} analyze spectral dependence.


More recently, scaling laws have been shown for kernel models under the Gaussian design, e.g. in \cite{Spigler_2020,cui2021generalization,Cui_2022} for regression and \cite{Cui_2023} for classification. 
\cite{maloney2022solvable} stud scaling laws for the random feature model in the context of regression. In the context of memorization for heavy-tailed data scaling laws have been shown in the infinite-memory setting \cite{hutter2021learning}, for ''quantized" skills \cite{michaud2023the} and for certain random data-generation processes \cite{debowski2023simplistic}. When taking model capacity and optimization into account, \cite{cabannes2023scaling} recently proved scaling laws in constraint-capacity associative memories.


To our knowledge, however, very few papers deal with the decay of scaling in the case of self-consuming loops. 

\julia{Do they show decay in scaling or rather just analyze iterative loops, regardless of scaling?} A notable example is \cite{bartlett2020neurips} which studies iterated retraining in the context of self-(knowledge-)distillation\julia{to be continued}




\paragraph{Emergence of ``skills" and scaling laws:}

Scaling laws give us an insight on bang-for-the-buck style trade-off for model training. However, cross-entropy loss is not a goal in and of itself: we want to train models that are endowed with a larger and larger skill set as we scale them up. For instance,  \cite{gordon-etal-2021-data} provide intuition and empirics for the scaling of BLEU score for MT with cross-entropy loss as $$BLEU(L) \approx Ce^{-kL},$$ demonstrating ``emergence" of good BLEU performance with scale. This type of ``emergence" has been massively confirmed in \cite{wei2022emergent}, where a working definition of ``emerging" is ``not present in smaller models, but appears in larger models". In this sense, \cite{wei2022emergent} demonstrate empirically a large number of ``skills" appearing with scale, like Multi-Task NLU, Modular arithmetic, word unscrambling and transliteration.

A theoretical model, providing an underpinning of the necessity of scaling laws for the emergence of skill has recently been given by \cite{arora2023theory}. They analyse ``emergence" with the scaling laws as a departure point in a model that links cross-entropy loss in LLMs to basic skills to show that scaling laws enable the model to learn (and generalize) efficiently. 

Strengthening the tie between scaling laws and emergent skill, albeit in the {\em opposite} direction, \cite{michaud2023the} posit that skills that emerge in ''quanta" imply a scaling law of the loss. Related, \cite{chen2023skillit} assume a hierarchy of skills to derive data curation mechanisms to precipitate the emergence of skills, though they do not allude to scaling laws directly.

 

==> grokking.tex <==
\section{Mitigating Model Collapse by Mixing with Good Data}
Here we explore the possibility of alleviating model collapse via the acquisition of even a tiny amount of data from the true data distribution, to complement AI polluted data (the wide web).
\subsection{Non-autoregressive Case}
\begin{theorem}[Grokking!]
Consider a sample of size $T$ of which a proportion $\pi$ comes from the true distribution $p$ and the remainder comes from a version $p'$ of $p$ with its tail chopped off at rank $k$. We have the following scaling laws for the Hutter LLM.

(A) \textbf{Early-Stage Dynamics.} For $T \ll k^\beta/\pi$, it holds that
\begin{eqnarray}
    E_{test} \asymp T^{-(1-1/\beta)} + k^{-(\beta-1)}.
\end{eqnarray}
Thus,  during this stage, the money spent on acquiring some clean data is not amortized!

(B) \textbf{Later-Stage Dynamics.} As soon as $ T \ge Ck^\beta/\pi $ (where $C$ is an absolute constant), it holds that
    \begin{eqnarray}
        E_{test} \asymp (\pi T)^{-(1-1/\beta)}.
    \end{eqnarray}
Thus, during this stage, we recover the unpolluted  sample-size law scaling $T^{-(1-1/\beta)}$, up to withing a multiplicative constant $\pi^{-(1-1/\beta)}$ (which can be seen as an increase in the price of data). For fixed $T$ and tunable $\pi$, this error rate scales like $\pi^{-(1-1/\beta)}$, which is yet another scaling law.
\label{thm:grokk}
\end{theorem}
\begin{figure*}[!h]
    \centering
    % \hspace{-1.65cm}
    \includegraphics[width=1.\textwidth]{err_vs_T_vs_pi_grokking.pdf}
    \vspace{-.75cm}
    \caption{Empirical Validation of Theorem \ref{thm:grokk}. The broken line corresponds to the $T^{-(1-1/\beta)}$ scaling law that would hold throughout in the absence of pollution. Notice the grokking behavior predicted by the theorem. For this experiment, the Zipf exponent of the true data distribution $p$ is $\beta=2$.}
    \label{fig:grokk}
\end{figure*}
Effectively, the above theorem predicts that for any fixed $\pi \in (0,1)$ (no matter how small), the test error grokks w.r.t sample size $T$. The result is empiricall confirmed in Figure \ref{fig:grokk}

\begin{remark}
Let us conclude this section by saying that clean data always helps, since $E_{test}$ is decreasing function of $\pi$. Indeed, from \eqref{eq:Epi}, the derivative w.r.T $\pi$ is $E_{test}'(\pi) = -T\sum_{i \ge k+1} p_i^2 (1-\pi p_i)^{T-1} \le 0$.
\end{remark}

\julia{Note: Should hold for bigram, autoregressive bigram and triplet in the same way. }

\julia{How does tail-curation help alleviate the grokking behaviour? In the same $k+\sqrt{k}$ way as before?}

\subsection{Grokking in the Case of Tail Narrowing}
\begin{theorem}[Grokking!]
Consider a sample of size $T$ of which a proportion $\pi$ comes from the true distribution $p=Zip(\beta)$ and the remainder comes from a version $p' = Zip(\beta')$. We have the following scaling law for the Hutter LLM,
\begin{eqnarray}
    E_{test} \asymp (\pi T)^{-c} + ((1-\pi) T^{-c'}),
\end{eqnarray}
where $c := (\beta-1)/\beta$ and $c' := (\beta-1)/\beta'$.

Define $\overline T := (\pi / (1-\pi))^{-a}$, where $a := s / (1-s)$, and $s := \beta/\beta'$. Then,

(A) \textbf{Early-Stage Dynamics.} For $T \lesssim \overline T$, it holds that
\begin{eqnarray}
    E_{test} \asymp ((1-\pi)T)^{-c'},
\end{eqnarray}
Thus,  if $\beta' > \beta$, then during this stage, the money spent on acquiring some clean data is not amortized!

(B) \textbf{Later-Stage Dynamics.} As soon as $ T \gtrsim \overline T $, it holds that
    \begin{eqnarray}
        E_{test} \asymp (\pi T)^{-c}.
    \end{eqnarray}
Thus, during this stage, we recover the unpolluted  sample-size law scaling $T^{-c}$, up to withing a multiplicative constant $\pi^{-c}$ (which can be seen as an increase in the price of data). For fixed $T$ and tunable $\pi$, this error rate scales like $\pi^{-c}$, which is yet another scaling law.
\label{thm:grokk2}
\end{theorem}

\subsection{Autoregressive Case}
\ElvisIssue{ (TODO) Include this later. One can predict that the bigram autoregressive case should  be the same non-autoregressive case.}

==> triplet.tex <==
\clearpage

\section{Capacity-Limited Memory Models: A Triplet Scaling Law}\label{sec:triplet2}

We now consider study model collapse phenomenon in  the context of the following simple associative memory model studied in \cite{cabannes2023scaling}
\begin{eqnarray}
\label{eq:eva}
\begin{split}
    f_T(i) &:= \arg\max_y H_T(i,y),\text{ where}\\
    H_T(i,y) &:= e_i^\top M_T u_y,\\
    M_T &:= \sum_i q_T(i) e_i u_{f_\star(i)}^\top \in \mathbb R^{d \times d}.
    \end{split}
\end{eqnarray}
This is a transformer-like finite-memory extension of 
 the infinite-memory model in \cite{hutter2021learning}. The integer $d \ge 1$ then plays the role of the "capacity" of the resulting model. Here, $f_\star:[N] \to [m]$ is an unknown function, for example, reduction modulo $m$, i.e $f_\star(i) := ((i-1)\text{ mod } m) + 1$; $q_T=q(\mathcal D_T)$ is probability distribution on $[N]$ which encodes an arbitrary learner, estimated using and iid sample $\mathcal D_t = \{(i_t,y_t) \mid t \in [T]\}$ of size $T$ collected from a probability distribution on $[N] \times [m]$, of the form
\begin{eqnarray}
    i \sim p = \mathrm{Zipf}(\beta),\quad y = f_\star(i).
\end{eqnarray}
The embedding vectors $e_1,e_2,\ldots e_N$ and $u_1,u_2,\ldots,u_m$ are a system of unit-vectors in $\mathbb R^d$, constructed so that the matrix $\mathbb R^{d \times d}$ remembers the input/output pairs $(i,j)$ it has seen, i.e $e_i^\top M u_{f_\star(i)} \approx q_T(i)$ if $(i,f_\star(i)) \in \mathcal D_T$. The weights $q_T(i)$ ensure that different memories are memorized faster than others.

\citet{cabannes2023scaling} proposed that iid random embeddings from the uniform distribution on the unit-sphere in $\mathbb R^d$ be used. In this setting, for different choices of $q$, the following general scaling law was established
\begin{eqnarray}
    E_{test} \asymp T^{-(1-1/\beta)} + d^{-c_q},
\end{eqnarray}
where the exponent $c_q \in (0,\infty)$ depends on $\beta$ and the algorithm $q$. For example, when $q$ encodes the counting measure $q_T(i) := n_T(i)/T$ (reminiscent of SGD), it was shown that $c_q = (1-1/\beta)/2 \in (0,1/2)$. Another algorithm  $q_T(i) := 1[n_T(i) \ge 1]/\sum_\ell 1[n_T(\ell) \ge 1]$ (remniscent of ADAM ) was proposed which attains a optimal error rate (over all algorithms based on random embeddings) with $c_q = \beta-1$.

In the context of model collapse which is the main focus of this manuscript, we have the following.
\begin{theorem}[Triplet Scaling Law]
For all the algorithms $q$ considered in \cite{cabannes2023scaling}, one has the following triplet scaling law w.r.t sample size $T$, embedding dimension $d$, and frequency cutoff $k$,
    \begin{eqnarray}
        E_{test} \asymp T^{-(1-1/\beta)} + d^{-c_q} + \textcolor{red}{k^{-(\beta-1)}}.
    \end{eqnarray}
    \label{thm:triplet}
% \ElvisIssue{Here we refer to }
\vspace{-0.7cm}
\end{theorem}
This result is empirically confirmed in Figure \ref{fig:tripletlaw}  and proved in Appendix \ref{app:triplet}.
%\yunzhen{Interpretation? After this scaling law, we will have the same loss of scaling, same grokking, and same n-scale?}


